NTUA-SLP at SemEval-2018 Task 1: Predicting Affective Content in Tweets with Deep Attentive RNNs and Transfer Learning

In this paper we present deep-learning models that submitted to the SemEval-2018 Task~1 competition: "Affect in Tweets". We participated in all subtasks for English tweets. We propose a Bi-LSTM architecture equipped with a multi-layer self attention mechanism. The attention mechanism improves the model performance and allows us to identify salient words in tweets, as well as gain insight into the models making them more interpretable. Our model utilizes a set of word2vec word embeddings trained on a large collection of 550 million Twitter messages, augmented by a set of word affective features. Due to the limited amount of task-specific training data, we opted for a transfer learning approach by pretraining the Bi-LSTMs on the dataset of Semeval 2017, Task 4A. The proposed approach ranked 1st in Subtask E "Multi-Label Emotion Classification", 2nd in Subtask A "Emotion Intensity Regression" and achieved competitive results in other subtasks.

==> tex/affective.tex <==
\section{Create affective features}
Starting from small manually annotated lexica, continuous norms (within the $[-1, 1]$ interval) for new words are estimated using semantic similarity and a linear model along ten affect-related dimensions (namely valence, dominance, arousal, pleasantness, anger, sadness, fear, disgust, concreteness, familiarity).
The method of generating word level norms is an extension of the model that was first proposed by \cite{malandrakis2013distributional} and relies on the assumption that given some metric of similarity between two words, one may derive the similarity between their affective ratings. This approach uses a set of $N$ words with known affective ratings, referred as seed words, as a starting point. More specifically, the affective rating of a word $w$ can be calculated as follows:

\begin{equation}
 \hat{\upsilon}(w) = \alpha_0+\sum_{i=1}^{N}\alpha_i\upsilon(t_i)S(t_i,w),\label{afmod}
\end{equation}
\noindent where $t_{1}...t_{N}$ are the seed words, $\upsilon(t_i)$ is the affective rating for seed word $t_i$, $\alpha_i$ is a trainable weight corresponding to seed $t_i$ and $S(\dot)$ stands for the semantic similarity metric between $t_i$ and $w$. 
 
The seed words $t_{1}$ are selected separately for each dimension, from the words available in
the original manual annotations (see \ref{annotations}). The $S(\dot)$ metric is estimated as shown in \cite{palogiannidi2015valence} using word-level contextual feature vectors and adopting a scheme based on mutual information for feature weighting.


\subsection{Manually annotated norms} \label{annotations}
In order to generate affective norms we need to start from some manual annotations. 
To that end we use ten dimensions from three sources. From the Affective Norms for English Words \cite{anew} we use norms for valence, arousal and dominance. From the MRC Psycholinguistic database \cite{coltheart1981mrc}, we use the
norms for concreteness and familiarity. From the Paivio norms \cite{clark2004extensions} we use
the norms for pleasantness. Finally from \cite{stevenson2007characterization} we use norms for anger, sadness, fear and disgust.

